How do Quadratic Regularizers Prevent Catastrophic Forgetting: The Role of Interpolation

Catastrophic forgetting undermines the effectiveness of deep neural networks (DNNs) in scenarios such as continual learning and lifelong learning. While several methods have been proposed to tackle this problem, there is limited work explaining why these methods work well. This paper has the goal of better explaining a popularly used technique for avoiding catastrophic forgetting: quadratic regularization. We show that quadratic regularizers prevent forgetting of past tasks by interpolating current and previous values of model parameters at every training iteration. Over multiple training iterations, this interpolation operation reduces the learning rates of more important model parameters, thereby minimizing their movement. Our analysis also reveals two drawbacks of quadratic regularization: (a) dependence of parameter interpolation on training hyperparameters, which often leads to training instability and (b) assignment of lower importance to deeper layers, which are generally the place forgetting occurs in DNNs. Via a simple modification to the order of operations, we show these drawbacks can be easily avoided, resulting in 6.2\% higher average accuracy at 4.5\% lower average forgetting. We confirm the robustness of our results by training over 2000 models in different settings. Code available at \url{https://github.com/EkdeepSLubana/QRforgetting}

==> collas (arxiv)/files/abstract.tex <==
\begin{abstract}
Catastrophic forgetting undermines the effectiveness of deep neural networks (DNNs) in scenarios such as continual learning and lifelong learning. While several methods have been proposed to tackle this problem, there is limited work explaining why these methods work well. This paper has the goal of better explaining a popularly used technique for avoiding catastrophic forgetting: quadratic regularization. We show that quadratic regularizers prevent forgetting of past tasks by interpolating current and previous values of model parameters at every training iteration. Over multiple training iterations, this interpolation operation reduces the learning rates of more important model parameters, thereby minimizing their movement. Our analysis also reveals two drawbacks of quadratic regularization: (a) dependence of parameter interpolation on training hyperparameters, which often leads to training instability and (b) assignment of lower importance to deeper layers, which are generally the place forgetting occurs in DNNs. Via a simple modification to the order of operations, we show these drawbacks can be easily avoided, resulting in 6.2\% higher average accuracy at 4.5\% lower average forgetting. We confirm the robustness of our results by training over 2000 models in different settings.
 \footnote{Code available at \url{https://github.com/EkdeepSLubana/QRforgetting}}
\end{abstract}

==> collas (arxiv)/files/conclusion.tex <==
\section{Conclusion}
In this work, we determine the mechanisms using which quadratic regularization based methods prevent catastrophic forgetting in DNNs. Our primary findings show that in the short-term, these methods interpolate current and past values of model parameters, disallowing change. In the long-term, they change the learning rate of a parameter in proportion to its importance, reducing the overall movement of more important parameters. Our analysis also shows two primary pitfalls that limit the effectiveness of quadratic regularization: (i) extrapolation, instead of interpolation, of parameters due to inappropriate hyperparameters and (ii) lower importance assignment to deeper layers. We propose an explicit interpolation variant of quadratic regularizers, which is able to circumvent these pitfalls, boasting much better performance, consistently. In future work, we aim to perform similar analyses of the mechanisms which allow replay-based techniques to prevent catastrophic forgetting.

\section*{Acknowledgements}
The authors thank Hidenori Tanaka and anonymous reviewers for valuable feedback on the paper. This work was supported in part by NSF under award CNS-2008151.

==> collas (arxiv)/files/emr_vs_qreg.tex <==
\begin{table}[t]
\caption{\label{tab:emr_vs_qreg}Comparison of Average Accuracy (Acc; $\uparrow$ indicates higher is better) and Average Forgetting (Forg; $\downarrow$ indicates lower is better) for plain and explicit interpolation variants of EWC, MAS, SI, and RWalk, averaged over five seeds (std.\ dev.\ are reported in appendix). Results are also provided with two replay based methods (A-GEM and ER-Reservoir) and plain fine-tuning (Plain). We consider three datasets: CIFAR-100 (10 tasks); Oxford-Flowers (17 tasks); and Caltech-256 (32 tasks). For a specific regularizer, the better performing variant is underlined; the best results are in bold. As shown, variants with explicit interpolation steps consistently outperform their Quadratic Regularization counterparts. This behavior is most prominent in datasets with unbalanced classes and longer task sequences (Oxford-Flowers and Caltech-256), where hyperparameter tuning is difficult.}
\tablefont
\begin{subtable}{\textwidth}
\centering
\begin{tabular}{@{}c!{\vrule width 1pt}c!{\vrule width 1pt}cccc|cc!{\vrule width 1pt}cccc!{\vrule width 1pt}cc@{}}
\toprule
\multicolumn{2}{c!{\vrule width 1pt}}{1 Epoch}     & \multicolumn{6}{c!{\vrule width 1pt}}{Plain Quadratic Regularizers}                                 & \multicolumn{4}{c!{\vrule width 1pt}}{Explicit Interpolation Variants} & \multicolumn{2}{c}{Replay} \\ \midrule
CIFAR   & Plain & EWC  & MAS  & SI   & RWalk                  & Van.\ & Rand.\  & EWC        & MAS                 & SI         & RWalk      & A-GEM & ER       \\ \midrule
Acc ($\uparrow$)    & 55.3  & 62.5 & 63.9 & 61.2 & {\ul 63.9} & 63.9 & 64.0 & {\ul 63.8} & {\ul 64.0} & {\ul 63.9} & 63.8       & 67.2 & \textbf{68.8}      \\
Forg ($\downarrow$)   & 9.13  & 2.07 & 0.56 & 3.20 & 0.54     & 0.24 & 0.12 & {\ul 0.08} & {\ul \textbf{0.06}} & {\ul 0.07} & {\ul 0.09} & 1.29 & 0.69 \\ \midrule
Flowers & Plain & EWC  & MAS  & SI   & RWalk      & Van.\       & Rand.\ & EWC & MAS                 & SI         & RWalk      & A-GEM & ER      \\ \midrule
Acc ($\uparrow$)    & 37.9  & 41.3 & 57.5 & 36.2 & 44.9       & 59.5 & 58.5 & {\ul 60.0} & {\ul 59.6}          & {\ul 59.9} & {\ul 59.4} & 68.61 & \textbf{68.9} \\
Forg ($\downarrow$)   & 13.4  & 10.6 & 3.61 & 15.1 & 9.68     & 1.19 & 3.61 & {\ul 1.03} & {\ul \textbf{0.44}}          & {\ul 0.99} & {\ul 1.31} & 4.08 & 3.45\\ \midrule
Cal-256 & Plain & EWC  & MAS  & SI   & RWalk      & Van.\       & Rand.\ & EWC   & MAS                 & SI         & RWalk      & A-GEM & ER      \\ \midrule
Acc ($\uparrow$)    & 40.1  & 41.9 & 53.7 & 40.9 & 43.7       & 55.1 & 56.3 & {\ul 56.2} & {\ul 57.3} & {\ul 56.0} & {\ul 55.8} & 63.9 & \textbf{64.3}\\
Forg ($\downarrow$)   & 6.21  & 5.59 & 3.92 & 5.68 & 4.69     & 1.89 & 1.59 & {\ul 1.41} & {\ul \textbf{0.36}} & {\ul 1.42} & {\ul 1.31} & 2.89 & 2.75 \\ \bottomrule
\end{tabular}
% \caption{\label{tab:emr_vs_qreg}1 epoch.}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{@{}c!{\vrule width 1pt}c!{\vrule width 1pt}cccc|cc!{\vrule width 1pt}cccc!{\vrule width 1pt}cc@{}}
\toprule
\multicolumn{2}{c!{\vrule width 1pt}}{30 Epochs}       & \multicolumn{6}{c!{\vrule width 1pt}}{Plain Quadratic Regularizers}                                 & \multicolumn{4}{c!{\vrule width 1pt}}{Explicit Interpolation Variants} & \multicolumn{2}{c}{Replay} \\ \midrule
CIFAR   				& Plain & EWC  & MAS  & SI   & RWalk    & Van.\ & Rand.\  		& EWC   & MAS   & SI          & RWalk & A-GEM & ER   \\ \midrule
Acc ($\uparrow$)    	& 60.7  & 63.6 & 66.3 & 62.8 & 64.7 	& 66.2  & 66.2 			& {\ul 66.3} 	& {\ul 66.0}  & {\ul 66.2} & {\ul 66.1}  & 66.4  & \textbf{66.8} \\
Forg ($\downarrow$)   	& 8.01  & 4.63 & 0.23 & 6.30 & 3.39     & 0.26  & 0.21 			& {\bf \ul 0.21} 	& {\ul 0.23}  & {\ul 0.25} & {\ul 0.29} & 3.10  & 1.64 \\ \midrule
Flowers 				& Plain & EWC  & MAS  & SI   & RWalk    & Van.\ & Rand.\ 		& EWC 	& MAS   & SI          & RWalk & A-GEM & ER   \\ \midrule
Acc ($\uparrow$)    	& 49.9  & 54.1 & 60.5 & 51.1 & 55.7     & 60.3  & 60.9 			& {\ul 61.3} 	& {\ul 61.6}  & {\ul 61.8} & {\ul 61.7}  & 68.9 & \textbf{69.4} \\
Forg ($\downarrow$)   	& 11.8  & 9.07 & 1.19 & 12.4 & 7.19     & \textbf{0.36}  & 1.79 			& {\ul 1.07} 	& {\ul 0.48}  & {\ul 0.62} & {\ul 0.71}  & 4.29  & 3.01 \\ \midrule
Cal-256 				& Plain & EWC  & MAS  & SI   & RWalk    & Van.\ & Rand.\ 		& EWC   & MAS   & SI          & RWalk & A-GEM & ER   \\ \midrule
Acc ($\uparrow$)    	& 40.6  & 50.3 & 60.1 & 50.6 & 53.7     & 60.0  & 60.1 			& {\ul 60.6} 	& {\ul 60.9}  & {\ul 60.8} & {\ul 60.6}  & 65.7  & \textbf{66.1} \\
Forg ($\downarrow$)   	& 15.8  & 7.15 & 0.99 & 7.41 & 4.69     & 0.32  & 0.22 			& {\ul 0.22} 	& {\ul \bf 0.18}  & {\ul 0.32} & {\ul 0.34}  & 2.86  & 2.32 \\ \bottomrule
\end{tabular}
% \caption{\label{tab:emr_vs_qreg_30epochs} 30 epochs.}
\end{subtable}
\end{table}



% \begin{table}[t]
% \tablefont
% \centering
% \caption{\label{tab:emr_vs_qreg}Comparison of Average Accuracy (Acc; $\uparrow$ indicates higher is better) and Average Forgetting (Forg; $\downarrow$ indicates lower is better) for plain and explicit interpolation variants of EWC, MAS, SI, and RWalk, averaged over five seeds (std.\ dev.\ are reported in appendix). Results are also provided with two replay based methods (A-GEM and ER-Reservoir) and plain fine-tuning (Plain). We consider three datasets: CIFAR-100 (10 tasks); Oxford-Flowers (17 tasks); and Caltech-256 (32 tasks). For a specific regularizer, the better performing variant is underlined; the best results are in bold. As shown, variants with explicit interpolation steps consistently outperform their Quadratic Regularization counterparts (average improvement in average accuracy: 6.2\%). This behavior is most prominent in datasets with unbalanced classes and longer task sequences (Oxford-Flowers and Caltech-256), where hyperparameter tuning is difficult.}
% \begin{tabular}{@{}c!{\vrule width 1pt}c!{\vrule width 1pt}cccc|cc!{\vrule width 1pt}cccc!{\vrule width 1pt}cc@{}}
% \toprule
% Dataset &       & \multicolumn{6}{c!{\vrule width 1pt}}{Plain Quadratic Regularizers}                                 & \multicolumn{4}{c!{\vrule width 1pt}}{Explicit Interpolation Variants} & \multicolumn{2}{c}{Replay} \\ \midrule
% CIFAR   				& Plain & EWC  & MAS  & SI   & RWalk    & Van.\ & Rand.\  		& EWC   & MAS   & SI          & RWalk & A-GEM & ER   \\ \midrule
% Acc ($\uparrow$)    	& 60.7  & 63.6 & 66.3 & 62.8 & 63.9 	& 66.2  & 66.2 			& {\ul 66.3} 	& {\ul 66.3}  & {\ul 66.2} & {\ul 66.1}  & 66.4  & \textbf{66.8} \\
% Forg ($\downarrow$)   	& 8.01  & 4.63 & 0.29 & 6.30 & 0.54     & 0.27  & 0.24 			& {\bf 0.21} 	& {\ul 0.23}  & {\ul 0.25} & {\ul 0.29} & 3.10  & 1.64 \\ \midrule
% Flowers 				& Plain & EWC  & MAS  & SI   & RWalk    & Van.\ & Rand.\ 		& EWC 	& MAS   & SI          & RWalk & A-GEM & ER   \\ \midrule
% Acc ($\uparrow$)    	& 49.9  & 50.7 & 61.5 & 49.4 & 44.9     & 60.3  & 61.9 			& {\ul 62.3} 	& {\ul 62.5}  & {\ul 61.8} & {\ul 61.7}  & 68.92 & \textbf{69.4} \\
% Forg ($\downarrow$)   	& 11.8  & 11.2 & 1.19 & 12.4 & 9.68     & \textbf{0.36}  & 1.79 			& {\ul 1.07} 	& {\ul 0.48}  & {\ul 0.62} & {\ul 0.71}  & 4.29  & 3.01 \\ \midrule
% Cal-256 				& Plain & EWC  & MAS  & SI   & RWalk    & Van.\ & Rand.\ 		& EWC   & MAS   & SI          & RWalk & A-GEM & ER   \\ \midrule
% Acc ($\uparrow$)    	& 40.6  & 50.3 & 60.1 & 50.6 & 43.7     & 60.0  & 60.1 			& {\ul 60.6} 	& {\ul 60.9}  & {\ul 60.8} & {\ul 60.6}  & 65.7  & \textbf{66.1} \\
% Forg ($\downarrow$)   	& 15.8  & 5.15 & 0.99 & 5.01 & 4.69     & 0.32  & 0.22 			& {\ul 0.22} 	& \textbf{0.18}  & {\ul 0.32} & {\ul 0.34}  & 2.86  & 2.32 \\ \bottomrule
% \end{tabular}
% \end{table}


==> collas (arxiv)/files/emr_vs_replay.tex <==
\begin{table}[t]
\tablefont
\centering
\caption{\label{tab:emr_vs_replay}Comparison of Average Accuracy (Acc; $\uparrow$ indicates higher is better) and Average Forgetting (Forg; $\downarrow$ indicates lower is better) for online augmented (labeled ``with DA'') EMR and Quadratic Regularization strategies (EWC, MAS, SI, RWalk, and Random) with Replay-based methods (A-GEM and ER-Reservoir). Due to space constraints, results for Vanilla regularizers are not provided. We consider three datasets: CIFAR-100 (10 tasks, labeled CIFAR); Oxford-Flowers (17 tasks, labeled Flowers); and Caltech-256 (32 tasks, labeled Cal-256). Best replay-based method's results are in bold. Best regularization-based method's results are underlined. As shown, the performance gap between online augmented EMR and replay-based methods is minimal. In contrast, \emph{existing} Quadratic Regularization strategies (except MAS) find it difficult to scale up when more updates are performed under online augmentation.}
\begin{tabular}{@{}c!{\vrule width 1pt}ccccc!{\vrule width 1pt}ccccc!{\vrule width 1pt}cc@{}}
\toprule
Dataset & \multicolumn{5}{c!{\vrule width 1pt}}{Quadratic Reg. (with DA)}         & \multicolumn{5}{c!{\vrule width 1pt}}{Explicit Movement Reg. (with DA)}                                 & \multicolumn{2}{c}{Replay} \\ \midrule
CIFAR   & EWC  & MAS  & SI   & RWalk & Rand & EWC        & MAS        & SI   & RWalk      & Rand       & A-GEM    & ER              \\ \midrule
Acc ($\uparrow$)    & 62.1 & 65.1 & 64.1 & 64.8  & 64.8 & 65.6       & {\ul 66.1} & 65.8 & 65.2       & 65.4       & 67.2     & \textbf{68.8}   \\
Forg ($\downarrow$)   & 4.68 & 1.04 & 8.22 & 0.86  & 0.27 & 0.40       & 0.46       & 0.53 & {\ul 0.21} & 0.23       & 1.29     & \textbf{0.69}   \\ \midrule
Flowers & EWC  & MAS  & SI   & RWalk & Rand & EWC        & MAS        & SI   & RWalk      & Rand       & A-GEM    & ER              \\ \midrule
Acc ($\uparrow$)    & 37.1 & 61.8 & 34.1 & 51.2  & 63.2 & 66.4       & 66.1       & 66.1 & 65.9       & {\ul 66.8} & 68.61    & \textbf{68.9}   \\
Forg ($\downarrow$)   & 22.1 & 4.72 & 18.1 & 12.5  & 2.42 & {\ul 0.68} & 1.31       & 1.15 & 1.34       & 0.81       & 4.08     & \textbf{3.45}   \\ \midrule
Cal-256 & EWC  & MAS  & SI   & RWalk & Rand & EWC        & MAS        & SI   & RWalk      & Rand       & A-GEM    & ER              \\ \midrule
Acc ($\uparrow$)    & 44.2 & 57.6 & 36.3 & 55.3  & 60.6 & 60.7       & {\ul 61.2} & 60.9 & 60.6       & 60.7       & 63.9     & \textbf{64.3}   \\
Forg ($\downarrow$)   & 8.42 & 2.97 & 13.3 & 4.10  & 0.89 & 0.45       & {\ul 0.16} & 0.47 & 0.54       & 0.48       & 2.89     & \textbf{2.75}   \\ \bottomrule
\end{tabular}
\end{table}

==> collas (arxiv)/files/experiments.tex <==
\subsection{Experimental Evaluation}
\label{sec:exptt_eval}
We now evaluate the effectiveness of the proposed quadratic regularizers with explicit interpolation steps. We also provide comparisons with two experience replay-based methods: A-GEM (\cite{agem}) and ER-Reservoir (\cite{er_reservoir}). We stress that our objective in reporting this comparison is \emph{not} to beat the state-of-the-art, but to evaluate if our modified quadratic regularizers can reduce the gap between regularization and replay based methods, which can be inappropriate for applications where long-term storage of training data undermines privacy or greatly increases cost (e.g., in embedded systems).

We use three datasets of different complexities: (i) CIFAR-100, divided into 10 tasks with 10 classes per task and 500 samples per class; (ii) Oxford-Flowers, divided into 17 tasks with 6 classes per task and 72 samples per class (on average); and (iii) Caltech-256, divided into 32 tasks with 8 classes per task and 95 samples per class (on average). Note that Oxford-Flowers and Caltech-256 have unbalanced classes and few samples per class, which are characteristics of several real-world applications. We use a 6-layer CNN for all datasets and train the model using SGD with momentum for all tasks; results for ResNet-18 are in the appendix. The first 3 tasks for all datasets are reserved to run a grid search for finding the optimal hyperparameter configuration (learning rate/regularization constant). Since the models are trained in the stable training regime (enforced via hyperparameter tuning), we train models for both 1 epoch, batch-size 10 setting advocated by \cite{gem} and 30 epochs, batch-size 256 setting where we find all models achieve 95--100\% training accuracy when training on a given task, ensuring convergence (an assumption made by prior work to derive their regularizer strategies). Further, following prior works (\cite{MAS, EWC, SI}), we use a multi-head setting. 

Results are shown in \autoref{tab:emr_vs_qreg}. We note explicit interpolation variants \emph{significantly} outperform plain quadratic regularizers. For ex., in the 1 epoch setting, \emph{accuracy improves by 6.2\% on average and up to 23\%.} We further make the following observations: (i) On unbalanced datasets and long task sequences, explicit interpolation results in substantial improvements. However, on CIFAR-100, whose tasks correspond to hundreds of parameter updates, plain quadratic regularizers perform competitively. This indicates when longer task sequences are used for hyperparameter search, the resulting configuration is able to perform well for subsequent tasks as well. In contrast, on Oxford-Flowers and Caltech-256, especially in the 1 epoch setting, where the respective tasks have only 43 and 76 parameter updates (on average), searching for adequate hyperparameters is difficult and plain quadratic regularizers result in up to 10\% forgetting. (ii) With our proposed modifications, quadratic regularizers achieve witness lower forgetting than replay based methods, but continue to underperform on average accuracy. However, we note that when long-term storage of training data is prevented by privacy or cost concerns, our modifications allow quadratic regularizers to serve as a useful and reliable alternative to replay based methods.

% \subsection{Regularization-Based vs.\ Replay-Based Methods}
% \label{sec:emr_vs_replay}
% Replay-based methods are well known to outperform regularization-based methods~\cite{er_reservoir}. With EMR, we are able to alleviate the problems related to training hyperparameters and biased importance definitions in quadratic regularization, resulting in consistently high performance compared to popular quadratic regularizers. However, even with these improvements, regularization-based methods still fall short of replay-based methods. 

% \input{files/emr_vs_replay}

% We address this problem using a straightforward solution: \emph{online data augmentation}. Specifically, every training iteration, instead of making an update only on the current batch of inputs, an update can also be made on an augmented version of the input. Here, \emph{online} implies samples from previous tasks are not stored for later replay by the model. For example, if horizontal flipping is the choice of augmentation, every time a batch is loaded, a flipped variant of the batch is also created. The model is updated on both the original and the flipped samples, and both batches are discarded immediately after their updates. For quadratic regularizers, this strategy is unlikely to perform well because more model updates generally result in more forgetting. In contrast, \autoref{tab:emr_vs_qreg} shows EMR experiences minimal forgetting in all settings, making it a good candidate for use with online data augmentation. % Talk about generalization-forgetting trade-off?

% To verify this claim, we compare online, horizontal-flip augmented EMR and quadratic regularization models with two replay-based methods: A-GEM \cite{agem} and ER-Reservoir \cite{er_reservoir}. A-GEM uses a buffer of samples from previous tasks to determine whether the current update is likely to result in forgetting. If so, it orthogonalizes the update with respect to gradient of buffer samples. ER-Reservoir maintains a buffer of samples from the previous tasks and for every update on the current task, also updates the model on a batch of randomly selected samples from the buffer. Replay-based strategies require at least two backpropagation steps--one on the buffer and one on the current task. By performing updates on both the current and augmented batches, online augmentation results in similar computational cost as replay-based methods, but does not require storage of samples from previous tasks.

% Results with online data augmentation are shown in \autoref{tab:emr_vs_replay}. These numbers can be compared with \autoref{tab:emr_vs_qreg}, where no augmentation was performed. We note the following:\vspace{-2pt}

% (i) Online data augmentation substantially reduces the difference between average accuracy achieved using EMR and replay-based methods. For example, on CIFAR-100, A-GEM is only 0.9\% better than EMR. \emph{We conclude when storage of samples from previous tasks is not possible, EMR with online data augmentation can be used to achieve high accuracy without forgetting previous tasks.}\vspace{2pt}\\
% (ii) Existing quadratic regularizers (except MAS) lose performance when online data augmentation is used. This indicates quadratic regularizers have difficulty scaling to more parameter updates. EMR does not suffer from this flaw and performs well with online data augmentation.

==> collas (arxiv)/files/explicitreg.tex <==
\section{Addressing Limitations in Quadratic Regularization}
\label{sec:emr}

Having established the mechanisms by which quadratic regularizers prevent catastrophic forgetting and the corresponding drawbacks of those mechanisms, we seek a simple way to avoid these problems and still prevent catastrophic forgetting. To this end, we note our analysis in \autoref{sec:limitations} shows that two primary conditions should be satisfied to ensure a quadratic regularizer performs well: (a) the regularizer should function in the interpolation regime and (b) importance scores be relatively constant across layers. We show these conditions can be easily satisfied by breaking the quadratic regularizer update (\autoref{eq:param_update}) into two operations:
\begin{equation} 
\label{eq:emr}
\begin{split}
&\text{(i)}\, \theta_{n} \to \theta_{n} - \eta \nabla_{\theta_{n}} L_{T_{n}} \quad\quad\quad \text{{\small (Task-specific change) \text{ and}}}\\
&\text{(ii)}\, \theta_{n} \to \left(1-R_{j}\right) \odot \theta_{n} + R_{j} \odot \theta_{n-1}^{*} \quad \text{{\small (Interpolation)}}.\\
\end{split}
\end{equation}
Here, the vector $R_{j}$ is defined to control the amount of interpolation at iteration $j$. Contrasting this update with the quadratic regularization update in \autoref{eq:param_update}, one can see the main difference lies in the order of operations: while quadratic regularizers perform the task-specific update and the interpolation operation \emph{in a single step}, our proposed modification breaks that update into \emph{two separate operations}. This makes the interpolation operation \emph{explicit}, instead of the implicit operation in quadratic regularization. .

To understand the benefit of making interpolation an explicit operation, notice that in \autoref{eq:emr}, \emph{the amount of interpolation is independent of the training hyperparameters}; only the vector $R_{j}$ controls the amount of interpolation. This allows us to circumvent the need of a regularization coefficient and helps avoid training instabilities arising from gradient descent dynamics (see \autoref{sec:lim1}). Further, we can exploit this independence to define $R_{j}$ in a manner such that the desired conditions for effective quadratic regularization are always satisfied. To this end, we define $R_{j}$ as a measure of the importance of a parameter for previous tasks relative to its importance for all tasks. Specifically, assume learning of the $n^{\text{th}}$ task is currently underway. Again using $\alpha_{n-1}$ to denote importance of parameters according to tasks $0$ to $n-1$ and $\alpha_{T_{n}}$ to denote the importance of parameters according to the $n^{\text{th}}$ task, we define the relative importance of a parameter $\theta_{n}^{(k)}$ as
\begin{equation} 
\label{eq:imp_ratios}
R_{j}^{(k)} = \frac{\sqrt{\alpha_{n-1}^{(k)}}}{\sqrt{\alpha_{T_{n}}^{(k)}} + \sqrt{\alpha_{n-1}^{(k)}}}.
\end{equation}
Here, the definition of importance of a parameter can be borrowed from any popular quadratic regularizer. Note that under this formulation, $R_{j}^{(k)}$ necessarily ranges from $0$ to $1$ for all parameters, hence satisfying condition (a) and ensuring stable training. If $R_{j}^{(k)}$ is large (closer to 1), then the $k^{\text{th}}$ parameter is relatively more important for preserving performance on previous tasks than for the current task. In this case, the parameter's \emph{previous} value is weighted more heavily to prevent its change. If $R_{j}^{(k)}$ is small (closer to 0), then the $k^{\text{th}}$ parameter is relatively less important for previous tasks. In this case, the parameter's \emph{current} value is weighted more heavily, allowing the parameter to adapt to a new task. Finally, we note that even if a parameter's absolute importance is low, its relative importance can be high if it is unimportant to previous tasks. \emph{Thus, using this definition for $R_{j}$, we can also avoid problems related to assignment of lower importance scores to deeper layers.}

We also add that the use of square root in \autoref{eq:imp_ratios} yields us small-but-significant improvements over use of simple magnitude ($\sim1$--$2$\% less forgetting, in general). To understand why, recall importance scores in our paper are computed in a running average manner. In a small-batch scenario (one of our primary setups), gradient noise is very high, especially in the early iterations (magnitude of order 100). This noise manifests as gradient spikes that produce large fluctuations in the current task's importance scores. Since the previously computed importance scores remain fixed and since we regularize the model using relative importance to previous tasks' importance scores, these gradient spikes bias learning towards the current task. To avoid this behavior, we use a sublinear function (square root) to minimize sensitivity to fluctuating scores. In fact, we found similar improvements with cube root too (another sublinear function). Over a few iterations, gradient noise is removed by the running average, thus improving signal to noise ratio and yielding reliable estimates. Thus, in the later iterations, both square root and magnitude show similar behavior. However, square root has better ability to avoid forgetting in the early iterations and hence its overall forgetting ends up being smaller.


\begin{algorithm}[tb]
   \caption{Quadratic Regularization with Explicit Interpolation Steps}
   \label{alg:emr}
\begin{algorithmic}
   \STATE {\bfseries Input:} parameterization $\theta_{n-1}^{*}$ and importance $\alpha_{n-1}$ after learning $n-1$ tasks; number of training iterations \#iters and Loss $L_{T_{n}}$ for learning the $n^{\text{th}}$ task.
   \STATE {\bfseries Initialize:} $\theta_{n} = \theta_{n-1}^{*}$; $\alpha_{T_{n}} = \mathbf{0}$.
   \FOR{$j=0$ {\bfseries to} \#iters-1}
   \STATE $\theta_{n} \to \theta_{n} - \eta \nabla_{\theta_{n}} L_{T_{n}}$ \hfill{\small (Task-specific change)}
   \STATE Update $\alpha_{T_{n}}$ %\hfill{\small (Task-specific importance)}
   \STATE Compute $R_{j} = \frac{\sqrt{\alpha_{n-1}}}{\sqrt{\alpha_{T_{n}}} + \sqrt{\alpha_{n-1}}}$ \hfill{\small (Relative importance)}              
   \STATE $\theta_{n} \to \left(1-R_{j}\right) \odot \theta_{n} + \left(R_{j}\right) \odot \theta_{n-1}^{*}$ \hfill{\small (Interpolation)}
   \ENDFOR
    \STATE $\alpha_{n} \to (\alpha_{T_{n}} + \alpha_{n-1})/2$ \hfill{\small (Update importance)}
   \STATE {\bfseries Return:} $\theta_{n}$, $\alpha_{n}$
\end{algorithmic}
\end{algorithm}

The overall algorithm for quadratic regularization with explicit interpolation steps is shown in \autoref{alg:emr}. Before proceeding, we highlight that instead of using our explicit update formulation, the dependence on hyperparameters could also have been removed by scaling down the regularization coefficient in standard quadratic regularizers with the model learning rate. However, this would still retain the presence of hyperparameters in the overall setup, in contrast with our explicit update formulation.



\input{files/emr_vs_qreg}

==> collas (arxiv)/files/intro.tex <==
\section{Introduction}
\label{sec:intro}
Learning algorithms are often designed under the assumption of independent and identical data distributions. However, this assumption is violated in several practical scenarios, such as continual learning and lifelong learning, where data distributions evolve constantly. In such settings, deep neural networks (DNNs) witness catastrophic forgetting and have difficulty adapting to new tasks without losing performance on previously learned ones. Several past works have tried to address this problem. For example, \cite{EWC, MAS, SI, RWalk} propose quadratic regularizers that penalize changes in parameters which are important for preserving performance on past tasks; \cite{er_reservoir, mer, er_grad, dgr} describe the use of memory buffers or generative models to fine-tune on samples from past tasks while learning new ones; and \cite{PNN, cl_nas, den} propose dynamic modification of network architecture to increase model capacity for accommodating new tasks. While these works have shown promising results, a detailed understanding of their proposed methods is still to be developed. Understanding the reasons due to which existing methods for preventing catastrophic forgetting work or fail can open the possibility of developing better methods. 

With this motivation, in this work, we analyze \emph{quadratic regularization}, a popular technique for preventing catastrophic forgetting in DNNs. Specifically, quadratic regularization based methods penalize changes in model parameters that are important for maintaining performance on previously learned tasks. For example, if $\theta_{n}$ denotes model parameters corresponding to the $n^{\text{th}}$ task, $T_{n}$, then the total training loss under quadratic regularization follows
\begin{equation}
\label{eq:loss}
L = L_{T_{n}} + \frac{\lambda}{2} \sum_{k} \alpha_{n-1}^{(k)} \left(\theta_{n}^{(k)} - \theta_{n-1}^{*(k)}\right)^{2},
\end{equation}
where $L_{T_{n}}$ is the $n^{\text{th}}$ task's loss, $\lambda$ is a regularization constant, $\theta_{n-1}^{*}$ is model parameterization at the end of $(n-1)^{\text{th}}$ task, $\alpha_{n-1}$ is the importance of parameters according to tasks $0$ to $n-1$, and $v^{(k)}$ indexes a vector $v$ at location $k$. Different methods define importance differently. For ex., \cite{MAS} define importance as the sensitivity of model output to changes in its parameters, while \cite{EWC} define importance as the diagonal of Fisher information matrix.

Beyond continual/lifelong learning and related applications, quadratic regularizers are often used for improving performance in transfer learning scenarios (\cite{finetune}). However, despite their clear importance, there is limited work explaining why quadratic regularizers reduce catastrophic forgetting (see \cite{raghu, taylor_reg} for notable exceptions). To bridge this gap, we analyze parameter updates under quadratic regularization and show it prevents forgetting by \emph{interpolating current values of model parameters and their values at the end of the previous task's training} (see \autoref{eq:param_update}). By unrolling this interpolation operation over multiple iterations, we further show that, \emph{in proportion to their importance, quadratic regularizers change the ``effective'' learning rate of a parameter} (\autoref{eq:unrolled}): learning rate of parameters that are more important to previously learned tasks is reduced, disallowing their change; meanwhile parameters that are less important are allowed to change relatively freely, allowing the model to accommodate new tasks.

Our analysis exposes two important drawbacks to using quadratic regularization for preventing catastrophic forgetting. (i) We find improper hyperparameter configurations can result in \emph{extrapolation}, instead of interpolation, of parameters (see \autoref{sec:quadreg}). This often leads to unstable training (see \autoref{sec:limitations}). (ii) To satisfy conservation properties associated with the hierarchical nature of DNNs (\cite{du, mechanics}), generally used importance definitions in quadratic regularization assign lower importance values to parameters in deeper layers (see \autoref{sec:limitations}). As recently shown by \cite{raghu}, forgetting in DNNs is primarily caused by changes to deeper layers' parameters. Thus, assignment of lower importance to deeper layers reduces the effectiveness of quadratic regularizers. Interestingly, both these limitations can be eliminated by breaking the update into two stages, thus making interpolation of parameters an explicit operation (see \autoref{sec:emr}).

\textbf{Main Contributions:} In this work, we analyze quadratic regularization based methods for mitigating catastrophic forgetting. We train more than 2000 models to verify our analysis. Our main contributions follow.
\begin{itemize}[leftmargin=*]
\item \textbf{Role of Interpolation in Quadratic Regularizers (\autoref{sec:quadreg}).} We analyze parameter updates under quadratic regularization and show that it interpolates current and past values of model parameters to prevent catastrophic forgetting at a given training iteration. Unrolled over multiple iterations, this interpolation operation reduces the effective learning rate of parameters that are more important for preserving performance on previously learned tasks. 
\item \textbf{Limitations in Quadratic Regularization (\autoref{sec:limitations}).} We identify two primary drawbacks in the formulation of quadratic regularization: (a) due to dependence of the interpolation operation on training hyperparameters, improper hyperparameter configurations often result in extrapolation of parameters (instead of interpolation), hence resulting in training instability and (b) assignment of lower importance to parameters in deeper layers, a consequence of the hierarchical nature of DNNs, makes it difficult for quadratic regularizers to prevent catastrophic forgetting. 
\item \textbf{Avoiding Limitations via Explicit Interpolation (\autoref{sec:emr}).} By making the interpolation operation explicit, we show training instability issues caused by sensitivity to training hyperparameters can be completely avoided. Further, we show that redefining importance scores relative to past tasks prevents catastrophic forgetting caused by inappropriate changes to deeper layer parameters. Overall, using these modifications enable quadratic regularizers to achieve 6.2\% higher average accuracy at 4.5\% lower average forgetting.
\end{itemize}

% Most successful methods for continual learning are based on replaying samples from previous tasks~\cite{er_reservoir, mer}. However, for privacy-sensitive or resource-constrained applications where storing data from past tasks may be prohibited or expensive, replay-based methods are infeasible. We therefore seek to improve the performance of data-independent solutions. To this end, we propose \emph{Explicit Movement Regularization (EMR)}, a continual learning algorithm that addresses the limitations in quadratic regularization by \emph{first} performing task-specific updates to learn the next task, and \emph{then} averaging model parameters with their previous values to prevent catastrophic forgetting. Through this disentanglement, \emph{EMR removes the impact of training hyperparameters on parameter interpolation}. Further, using a measure of relative importance of a parameter for previous versus current tasks, \emph{EMR also avoids issues related to use of biased importance definitions for parameter interpolation}. Compared to quadratic regularization, EMR attains 6.2\% higher average accuracy at 4.5\% lower average forgetting. Using online data augmentation, without storing samples from previous tasks, EMR also performs competitively with replay-based methods.

==> collas (arxiv)/files/limitations.tex <==
\subsection{Limitations in Quadratic Regularization}
\label{sec:limitations}
Having elucidated the role of parameter interpolation in the effectiveness of quadratic regularizers, we now show how the dependence of this operation on the product $\eta \lambda \alpha^{(k)}$ introduces several drawbacks. We intentionally interleave our analysis with experimental evidence to show our claims hold well in practice. 

\setlength{\intextsep}{0pt}%
\begin{wrapfigure}{R}{6cm}
\begin{center}
\includegraphics[width=\linewidth, scale=1]{images/neg_heatmap_cifar.pdf}
\end{center}
\caption{\textbf{Case 1: $\eta \lambda \alpha_{n-1}^{(k)} < 0$. Negative importance scores lead to unstable training.} Green, outlined (red) cells imply stable (unstable) training. We analyze a 6-layer CNN trained using SI on 10 CIFAR-100 tasks. \emph{Original} implies both positive and negative scores are allowed, \emph{All Pos.} implies all scores are positive, and \emph{0.1\% Neg.} implies only 0.1\% of parameters are allowed negative scores. Average accuracy is noted inside figure cells (random accuracy=$10\%$, since any given task has 10 classes; plain fine-tuning accuracy=$55.2\%$). Training is always stable when all scores are positive. However, allowing even a few negative scores produces unstable training. A small $\lambda$ mitigates this behavior, but reduces the regularizer's effectiveness, resulting in similar performance to plain fine-tuning. Results on other datasets are provided in the appendix.\vspace{-5pt}}
\label{fig:negmap}
\end{wrapfigure}

\textbf{Setup:} We study four widely used quadratic regularizers: \emph{EWC} (\cite{EWC}), \emph{MAS} (\cite{MAS}), \emph{SI} (\cite{SI}), and \emph{RWalk} (\cite{RWalk}). Training without any strategy to mitigate catastrophic forgetting is called \emph{plain fine-tuning}. We use a 6-layer CNN trained using SGD at a fixed learning rate ($\eta$) of 0.001 on CIFAR-100 tasks (10 tasks; 10 classes per task). This is similar to architectures used in prior work: \cite{SI} use a 6-layer model (4 convolutional+2 dense layers); \cite{RWalk} use a 5-layer model (4 convolutional+1 dense layer); \cite{MAS} use AlexNet (5 convolutional+3 dense layers). We define training as \emph{unstable} if loss proceeds towards infinity, yielding out of precision (\emph{NaN}) gradients and parameters. Our experiments in \autoref{sec:lim1} follow the 1 epoch, batch-size 10 setting advocated by \cite{gem}, who argue that for lifelong learning problems, the model should be allowed to see a sample only once. We highlight that training instabilities elucidated in this section emerge in the first few training iterations themselves ($<$10, generally); hence, these results are not sensitive to the number of epochs. Our analysis in \autoref{sec:lim2} trains model in the stable training regime, where number of epochs can matter. We thus provide results for both 1 epoch, batch-size 10 and 30 epochs, batch-size 256 setting. We find our results follow the same qualitative patterns for both settings. Results are reported on the following metrics (\cite{RWalk}): (a) \emph{average accuracy}, defined as average test accuracy achieved by the final model over all tasks, and (b) \emph{average forgetting}, defined as the average amount of forgetting over all tasks, where an individual task's forgetting is described as the difference between the maximum and final accuracy achieved on it. All results are averaged over five seeds; standard deviations are reported as error bars in figures. For results on other datasets, see appendix.

\subsubsection{Extrapolation and Training Instability}
\label{sec:lim1}
For the $k^{\text{th}}$ parameter, the interpolation operation at every training iteration follows: $\left(1 - \eta \lambda \alpha_{n-1} \right) \odot \mathbf{\theta}_{n}^{(k)} + \left(\eta \lambda \alpha_{n-1} \right) \odot \mathbf{\theta}_{n-1}^{*(k)}$. Since there are generally no constraints on the training hyperparameters and since the scale of importance values can be arbitrarily large or small (e.g., see \autoref{fig:imp_scale}), it is possible for the value of $\eta \lambda \alpha^{(k)}$ to become either negative or greater than 1. In both cases, the interpolation operation converts into an \emph{extrapolation} operation. In this extrapolation regime, we find quadratic regularizers witness unstable training and severe performance degradation. 

\textbf{Case 1.} $\eta \lambda \alpha_{n-1}^{(k)} < 0$.
For parameters with negative importance, the value of $1 - \eta \lambda \alpha_{n-1}^{(k)} > 1$. This pushes the regularizer to the extrapolation regime for such parameters. To understand the implications of this setting, recall the learning rate of a parameter is multiplied by exponents of $1 - \eta \lambda \alpha_{n-1}^{(k)}$ (see \autoref{eq:unrolled}). This implies, for finite gradient, \emph{parameters with negative importance will experience exponentially large updates}, resulting in unstable training. 

To experimentally test this claim, we analyze SI, which allows negative importance scores to be assigned to a parameter. We use SI to train models for different values of $\lambda$ with a fixed learning rate of 0.001. We compare three cases: (a) the original method, which allows both positive and negative scores; (b) using absolute values of the assigned importance scores, thus ensuring all parameters have positive scores; and (c) using absolute values of the importance scores for all but 0.1\% randomly picked, negative importance parameters, hence allowing a very small number of negative scores. The results are shown in \autoref{fig:negmap} and lead to the following observations. (i) When only positive scores are allowed, training remains stable and the final model achieves high average accuracy. (ii) The original method, which allow both positive and negative scores, results in unstable training. In fact, allowing even a few negative scores leads to unstable training. For a very small value of $\lambda$, we note that this behavior is partially mitigated. This can be attributed to the fact the exponent's base, $1 - \eta \lambda \alpha_{n-1}^{(k)}$, remains approximately 1 for small $\lambda$. However, for this setting, the amount of interpolation is very low and hence the effectiveness of quadratic regularization is reduced, resulting in similar performance to plain fine-tuning.

The above experiment corroborates our claim that for negative importance scores, training becomes unstable. This result also shows that \emph{importance scores should be positive for all parameters.} This raises the question, why does SI work well? Interestingly, we find that even though in their paper the authors propose SI as a signed method (i.e., negative scores are allowed) and derive theoretical results for such a signed importance setting, their implementation actually uses a rectifier function (ReLU) to remove negative scores during training (\cite{sigit}). This detail is not discussed in the paper and is likely why the method works well in practice. 

\begin{figure}
\centering
\centerline{\includegraphics[width=\columnwidth]{images/icml_vios_together.pdf}}
\caption{\textbf{Case 2: $\eta \lambda \alpha_{n-1}^{(k)} > 1$. Percentage of parameters that violate $\eta \lambda \alpha_{0}^{(k)} < 1$, leading to unstable training.} We use different values of $\lambda$ to train a 6-layer CNN on CIFAR-100 tasks. We include results with and without clamping of importance scores, which enforces the constraint that $\eta \lambda \alpha_{0}^{(k)} \le 1$ for all parameters. A dotted line marks $\lambda$ at which $\eta \lambda \alpha_{n-1}^{(k)} = 1$ for just one parameter--we first expect to see unstable training right after this value. Green (Red) shading implies we expect training to be stable (unstable) for the corresponding $\lambda$. As shown, across 1.2 million parameters, with even a few violations, training becomes unstable: 5 (0.0004\% parameters) for EWC, 26 (0.002\% parameters) for MAS, 12 (0.001\% parameters) for SI, 31 (0.002\% parameters) for RWalk. The use of clamping helps avoid this instability and yields good performance, indicating the violating parameters were the cause for training instability. Results on other datasets are provided in the appendix.}
\label{fig:violations}
\end{figure}


\textbf{Case 2.} $\eta \lambda \alpha_{n-1}^{(k)} > 1$.
Note that if $\eta \lambda \alpha_{n-1}^{(k)} > 1$ for a parameter, the value of $1 - \eta \lambda \alpha_{n-1}^{(k)} < 0$ for it. That is, similar to Case 1, the regularizer is again pushed into the extrapolation regime. Since $1 - \eta \lambda \alpha_{n-1}^{(k)}$ is multiplied to the current parameter value at every iteration (see \autoref{eq:param_update}), for a reasonably high value of the parameter (i.e., greater than the gradient), we see the parameter's \emph{sign will be flipped (changed) every update}, resulting in unstable training. 

To demonstrate this claim, we train models using different quadratic regularizers and calculate the number of parameters that violate the inequality $\eta \lambda \alpha_{0}^{(k)} < 1$ (i.e., after first task) for various regularization constants. As shown in \autoref{fig:violations}, training is \emph{always} stable when $\lambda$ is small enough to ensure the inequality is not violated. However, with even a \emph{few} violations (\emph{$<$4--30 out of 1.2 million parameters}), training becomes unstable. To confirm that it is indeed these few violating parameters that cause instability, we also include results with a ``clamping'' operation, which enforces the constraint $\eta \lambda \alpha_{0}^{(k)} \le 1$ for all parameters by reassigning violating parameters an importance score of $\nicefrac{1}{\eta\lambda}$. As can be seen in the figure, the clamped models do not witness any instability and are able to achieve high performance. 

Combined, these results corroborate our claim that if $\eta \lambda \alpha_{n-1}^{(k)} > 1$, training becomes unstable. We stress that even though the clamping operation in the experiments above helps address unstable training, its imposed constraint of $\eta \lambda \alpha_{n-1}^{(k)} = 0$ will yield an effective learning rate of $0$ for violating parameters  (see \autoref{eq:vec_update2}). This implies such parameters will be frozen at their current value and not allowed to change. Consequently, if an overly large $\lambda$ is used, a significant portion of the model may remain frozen, disallowing learning of new skills. 

Overall, the above two cases complete our analysis of training instability in the extrapolation regime. Experimentally, we find that as long as the regularizer is in the interpolation regime, training remains stable. In fact, during hyperparameter tuning, we recommend the constraint $0 < \eta \lambda \alpha_{n-1}^{(k)} < 1$ for all parameters should be used to reject values of $\eta$ and $\lambda$ that are likely to produce unstable training.

\subsubsection{Disparate Importance Assignment}
\label{sec:lim2}

% \begin{figure}
% \centering
% \centerline{\includegraphics[width=\columnwidth]{images/icml_imp_together.pdf}}
% \caption{\textbf{Average importance is lower for parameters in deeper layers.} We train a 6-layer CNN on the first CIFAR-100 task and analyze importance definitions used by popular quadratic regularizers. As shown, except for SI, importance definitions used in quadratic regularizers result in much lower average importance for parameters in deeper layers. See appendix for results on other datasets.}
% \label{fig:imp_scale}
% \end{figure}

\setlength{\intextsep}{0pt}%
\begin{wrapfigure}{R}{6cm}
\begin{center}
\includegraphics[width=\linewidth, scale=1]{images/icml_imp_together.pdf}
\end{center}
\caption{\textbf{Average importance is lower for parameters in deeper layers.} We train a 6-layer CNN on the first CIFAR-100 task and analyze importance definitions used by popular quadratic regularizers. As shown, except for SI, importance definitions used in quadratic regularizers result in much lower average importance for parameters in deeper layers. Results on other datasets are provided in the appendix.}
\label{fig:imp_scale}
\end{wrapfigure}

We find that importance definitions used in popular regularizers can assign (much) lower importance to deeper layers than to earlier layers (e.g., see results for EWC in \autoref{fig:imp_scale}). This phenomenon can be explained by borrowing a result from the field of network pruning, where similar importance definitions are used for removing unnecessary parameters in DNNs (\cite{shrinkbench}). Specifically, due to rescale symmetry in DNNs with ReLU non-linearities, layerwise norms of model parameters are conserved across a model (\cite{du, mechanics}). \cite{synflow} recently show that to satisfy this property, generally used importance definitions assign much lower importance to parameters in deeper layers than to parameters in earlier layers. 

% \setlength\intextsep{0pt}
% \begin{wrapfigure}{R}{7.5cm}
% \centering
% \includegraphics[width=\linewidth, scale=1]{cka_analysis.png}
% \caption{\textbf{Balanced importance scores prevent forgetting more effectively.} We use CKA to measure representational similarity between layers of a model trained only on the first task of CIFAR-100 versus the model trained on all tasks. Average accuracy (Acc.) and average forgetting (Forg.) are reported in the legend. Unlike other methods, Vanilla and Random are not biased against deeper layers; they achieve high representational similarity across all layers with minimal forgetting. In contrast, the other measures have significantly lower CKA similarity in deeper layers and, hence, witness more forgetting. Results on other datasets are provided in the appendix.}
% \label{fig:cka_analysis}
% \end{wrapfigure}
\begin{figure}
\begin{subfigure}{.5\textwidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth]{images/cka_analysis_1epoch.pdf}}
  \caption{1 epoch.}
  \label{fig:1epochs}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth]{images/cka_analysis_30epochs.pdf}}
  \caption{30 epochs.}
  \label{fig:30epochs}
\end{subfigure}
\caption{\textbf{Balanced importance scores prevent forgetting more effectively.} We use CKA to measure representational similarity between layers of a model trained only on the first task of CIFAR-100 versus the model trained on all tasks. Average accuracy (Acc.) and average forgetting (Forg.) are reported in the legend. Balanced variants ensure importance scores are not biased against deeper layers; they achieve high representational similarity across all layers with minimal forgetting. In contrast, the other measures have significantly lower CKA similarity in deeper layers and, hence, witness more forgetting. Results on other datasets are provided in the appendix.}
\label{fig:cka_analysis}
\end{figure}

To understand the implications of this disparate importance assignment, recall that for stable training, the constraint $\eta \lambda \alpha_{n-1}^{(k)} < 1$ must be satisfied for all parameters. Thus, assuming stable training and a given value of $\eta$, the regularization constant ($\lambda$) will be bounded as follows:
\begin{equation}
\label{eq:lambda_upper}
\lambda < \lambda_{\text{upper}} = \min_{k} \left[\frac{1}{\eta \, \alpha_{n-1}^{(k)}}\right] = \frac{1}{\eta\,\max_{k} \alpha_{n-1}^{(k)}}.
\end{equation}
\autoref{eq:lambda_upper} shows that under stable training, \emph{the valid range for $\lambda$ is restricted by the largest importance score assigned to a model parameter}. However, given the disparate importance assignment in popular quadratic regularizers, will this range be suitable for all parameters in a model? To understand this, we note for a general parameter $\theta_{n}^{l}$, the value of $\eta \lambda \alpha_{n-1}^{(l)}$ is bounded as follows:
\begin{equation}
\label{eq:ratio}
\eta \lambda \alpha_{n-1}^{(l)} < \eta \lambda_{\text{upper}} \alpha_{n-1}^{(l)} = \frac{\alpha_{n-1}^{(l)}}{\max_{k} \alpha_{n-1}^{(k)}}.
\end{equation}
If $\alpha_{n-1}^{(l)} \ll \max_{k} \alpha_{n-1}^{(k)}$, \autoref{eq:ratio} shows the product $\eta \lambda \alpha_{n-1}^{(l)} \to 0$. Thus, \emph{regardless of how large the value of $\lambda$ is}, we find parameters with relatively lower importance will be permitted to change rapidly during training, enabling the model to learn new tasks. Indeed, this is the desired behavior. \emph{However}, in the context of DNNs, we have shown standard importance definitions in quadratic regularizers can assign much lower importance to deeper layers (see \autoref{fig:imp_scale}). This indicates \emph{currently used quadratic regularizers will allow a model to change its deeper layers more readily than its earlier layers}. As shown by \cite{raghu}, forgetting in DNNs is primarily caused by adaptation of deeper layers to recent tasks. Thus, by using lower importance scores for parameters in deeper layers, quadratic regularizers are unable to address the primary source of catastrophic forgetting in DNNs: changes to deeper layers. 

Our analysis above also indicates treating deeper layers on the similar scale of importance as earlier layers should allow a quadratic regularizer to prevent forgetting more easily. To experimentally test this, we design quadratic regularizers with balanced importance assignments across layers. This is achieved via rescaling layerwise importance scores, such that the average importance of scores in any layer is the same. We also consider two naive baselines that satisfy this constraint: (a) \emph{Vanilla}--assign unit importance to all parameters, and (b) \emph{Random}--assign uniformly picked, random importance between $[0, 1]$ to all parameters. Following \cite{raghu}, we analyze each layer's contribution to catastrophic forgetting by using Centered Kernel Alignment (CKA) (\cite{CKA}) and evaluate similarity of feature representations between a model trained only on the first task and a model trained on all tasks. If forgetting is low, features are similar and CKA is high across all layers of the two models. We use the first 3 tasks of our CIFAR-100 setup to perform a hyperparameter search for $\lambda$. The remaining 7 tasks are used for training and evaluation. We train models for both 1 epoch with a batch-size of 10 and 30 epochs with a batch-size of 256. Results are shown in \autoref{fig:cka_analysis}. As can be seen, models trained using balanced quadratic regularizers forget the least and have comparable average accuracy. CKA similarity is high across all layers. In contrast, methods with disparate importance assignment forget more and show low CKA similarity in deeper layers. The above experiment corroborates our claim that \emph{catastrophic forgetting is better prevented by assigning similar importance to all layers, than by using existing, more complex importance definitions.} Surprisingly, prior work on quadratic regularization generally do not evaluate their methods against such simple baselines like Vanilla and Random. \footnote{We note that \cite{EWC} do have a comparison to distance based regularization, which is similar to our Vanilla technique, but their results are for a setting where one computes and stores importance scores computed after every task. This yields a memory complexity that is proportional to the product of model size and number of tasks, ignoring one of the core desiderata of continual learning that memory requirements should grow at most sub-linearly with the number of tasks (\cite{thesis}).}

==> collas (arxiv)/files/quadreg.tex <==
\section{The Role of Interpolation in Quadratic Regularization}
\label{sec:quadreg}
We first establish notations used throughout the paper. $\theta_{n}$ denotes model parameters and $L_{T_{n}}$ denotes a task-specific loss for the $n^{\text{th}}$ task; $\theta_{n-1}^{*}$ denotes model parameters at the end of task $n-1$; $\eta$ denotes the learning rate; and $\lambda$ denotes the regularization constant. We use $v^{(k)}$ to index a vector $v$ at location $k$. To match the empirical setup in which quadratic regularizers generally function, we assume importance scores for regularizing the $n^{\text{th}}$ task (denoted $\alpha_{n-1}$) are calculated during training of tasks $0$ to $n-1$. These scores stay constant as the $n^{\text{th}}$ task proceeds. The total loss for learning the $n^{\text{th}}$ task follows \autoref{eq:loss}.
% \begin{equation}
% \label{eq:loss}
% L = L_{T_{n}} + \frac{\lambda}{2} \sum_{k} \alpha_{n-1}^{(k)} \left(\theta_{n}^{(k)} - \theta_{n-1}^{*(k)}\right)^{2}.
% \end{equation}

Our analysis into the mechanics of quadratic regularization is based on a decomposition of the parameter updates. Specifically, computing the gradient of \autoref{eq:loss}, we see the parameter vector, $\theta_{n}$, updates as follows:
\begin{equation}
\label{eq:vec_update}
\theta_{n} \to \theta_{n} - \eta \left(\nabla_{\theta_{n}} L_{T_{n}} + \lambda \alpha_{n-1} \odot \left(\theta_{n} - \theta_{n-1}^{*}\right) \right).
\end{equation}
Rearranging \autoref{eq:vec_update}, we see the $k^{th}$ model parameter updates as follows:
\begin{equation}
\label{eq:param_update}
\theta_{n}^{(k)} \to \underbrace{\left(1 - \eta \lambda \alpha_{n-1}^{(k)}\right) \theta_{n}^{(k)} + \left(\eta \lambda \alpha_{n-1}^{(k)}\right) \theta_{n-1}^{*(k)}}_{\text{Interpolation b/w current and previous values }} \underbrace{- \eta \frac{\partial L_{T_{n}}}{\partial\theta_{n}^{(k)}}.}_{\text{Task Derivative}}
\end{equation}
The above equation illustrates that under quadratic regularization, \emph{a new task is learned by moving model parameters along task-specific derivatives}, while forgetting of previously learned tasks is prevented by \emph{simultaneously performing an interpolation operation between current and previous values of model parameters}. Essentially, the interpolation operation minimizes drift of important model parameters, thus ensuring one can retain performance on previously learned tasks while learning new ones. To understand how mere interpolation of parameters can help mitigate catastrophic forgetting over multiple iterations, we derive the total change in model parameters between the ($n$-1)$^{\text{th}}$ and the $n^{\text{th}}$ tasks. Specifically, if the task-specific gradient for the $j^{\text{th}}$ training iteration is denoted as $g_j$, then unrolling the parameter updates in \autoref{eq:param_update} via recursive substitution for $i$ iterations yields:
\begin{equation}
\label{eq:unrolled}
\theta_{n}^{(k)} = \theta_{n-1}^{*(k)} - \sum_{j = 0}^{i-1} \underbrace{\left[\left(1 - \eta \lambda \alpha_{n-1}^{(k)}\right)^{i-j-1}\eta \right]}_{\text{Effective Learning Rate}} g_{j}^{(k)}.
\end{equation}
\autoref{eq:unrolled} shows that, \emph{based upon its importance, quadratic regularizers change the learning rate of a parameter}. In particular, the effective learning rate at which the $k^{\text{th}}$ parameter updates is calculated by multiplying $\eta$ with exponents of $1 - \eta \lambda \alpha_{n-1}^{(k)}$. If the parameter’s importance is high, the value of $1 - \eta \lambda \alpha_{n-1}^{(k)}$ becomes smaller, consequently reducing the parameter's learning rate and restricting its change. If the parameter’s importance is low, the value of $1 - \eta \lambda \alpha_{n-1}^{(k)}$ remains essentially unchanged; consequently, the parameter's effective learning rate is approximately equal to $\eta$, allowing it to freely change according to task derivatives and enable learning of new tasks.

Overall, \autoref{eq:param_update} and \autoref{eq:unrolled} establish the exact mechanisms by which quadratic regularizers help mitigate catastrophic forgetting. Specifically, \autoref{eq:param_update} shows that in the short-term, quadratic regularizers use a weighted interpolation of model parameters with their previous values to prevent changes to important parameters. Meanwhile, \autoref{eq:unrolled} shows that, in the long-term, quadratic regularizers reduce the learning rate of important parameters, slowing their change as new tasks are learned. These mechanisms alter a model’s optimization path, allowing unimportant parameters to adapt and accommodate new tasks, while restricting movement of important parameters to retain performance on previously learned tasks and prevent catastrophic forgetting. We also note that since the weights used in parameter interpolation (\autoref{eq:param_update}) depend on the product of the learning rate ($\eta$), the regularization constant ($\lambda$), and the parameter’s importance ($\alpha^{(k)}$), essentially these three variables determine the effectiveness of a regularizer.



==> collas (arxiv)/files/related.tex <==
\section{Related Work}
\label{sec:related}

Several prior works have proposed solutions to the problem of catastrophic forgetting in DNNs. Due to their higher relevance to our work, we focus on quadratic regularization based methods in this section. Detailed discussion of other techniques is provided in the appendix. 

\textbf{Quadratic Regularization Based Methods:} \cite{EWC} developed Elastic Weight Consolidation (EWC), a quadratic regularization strategy that defines the importance of model parameters using the diagonal of the Fisher information matrix. Since EWC, several quadratic regularizers have been proposed. For ex., \cite{SI} describe Synaptic Intelligence (SI), which defines a parameter's importance as the contribution of that parameter to reduction in loss for previous tasks; \cite{ritter} replace EWC's diagonal Fisher approximation with a block-diagonal Hessian approximation; \cite{MAS} describe Memory Aware Synapses (MAS), for which a parameter's importance is defined as the sensitivity of model output to change in that parameter; and \cite{RWalk} describe Riemannian Walk (RWalk), which defines a parameter's importance as the sum of the diagonal of the Fisher information matrix and the contribution of that parameter to reduction in loss for previous tasks. 

\textbf{Understanding Methods for Mitigating Catastrophic Forgetting:} A few papers have sought to understand the reasons behind catastrophic forgetting and the effectiveness of existing methods for alleviating it (\cite{genforget, regimes, lmc, ntk, nphard, ogd_guarantees}). We specifically highlight an important relevant work by \cite{raghu}, who use Centered Kernel Alignment (CKA) (\cite{CKA}) to measure representational similarity between models trained on different numbers of tasks. The authors demonstrate that catastrophic forgetting primarily arises due to adaptation of deeper layers to new tasks. Solutions that prevent catastrophic forgetting minimize this adaptation, thus ensuring the model can perform well on both novel and previously learned tasks. Closely related to our work is also the recent paper by \cite{taylor_reg}, who analyze quadratic regularizers by focusing on their asymptotic properties (i.e., convergence and generalization behavior). Similarly, \cite{benzing} discusses how different importance defintions in popular quadratic regularizers are related to each other via different approximations of the Fisher information matrix. In contrast to these papers, we focus on the model updates themselves: our work aims to understand limitations in quadratic regularization methods arising from its gradient descent dynamics. As we show, an implicit interpolation operation helps QR methods prevent catastrophic forgetting, and its interplay with training hyperparameters yields clear regimes of training instability in QR methods. We also note that some prior works have proposed Bayesian perspectives for understanding and improving quadratic regularization techniques by introducing better importance definitions (\cite{huszar, EWC, ritter}), however these works often make strong assumptions that are unlikely to hold in practice, such as assuming the model gradient remains zero for previous tasks (to allow a Laplace or second-order Taylor’s approximation). In contrast, our work makes no assumptions about the model’s capabilities for solving a prior task, using the exact dynamics equations. 

% We do note the suggested paper [4] empirically observes model parameters can witness exploding gradients under QR. Our work provides the exact theoretical reason behind this observation. 

==> collas (arxiv)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> collas (arxiv)/title.tex <==
\author{%
  Ekdeep Singh~Lubana\\
  \texttt{eslubana@umich.edu} \\
  \And
  Puja Trivedi \\
  \texttt{pujat@umich.edu} \\
  \And
  Danai Koutra \\
  \texttt{dkoutra@umich.edu} \\
  \And
  Robert P.\ Dick \\
  \texttt{dickrp@umich.edu} \vspace{5pt}\\
  EECS Department\\
  University of Michigan\\
  }


% Authors must not appear in the submitted version. They should be hidden
% as long as the \collasfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.

\author{Ekdeep Singh Lubana, Puja Trivedi, Danai Koutra, \& Robert P. Dick \\
EECS Department\\
University of Michigan, Ann Arbor\\
USA \\
\texttt{\{eslubana, pujat, danaik, dickrp\}@umich.edu} \\
}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to \LaTeX{} to determine where to break
% the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% puts 3 of 4 authors names on the first line, and the last on the second
% line, try using \AND instead of \And before the third author name.


==> files/emr_vs_replay.tex <==
\begin{table}[t]
\tablefont
\centering
\caption{\label{tab:emr_vs_replay}Comparison of Average Accuracy (Acc; $\uparrow$ indicates higher is better) and Average Forgetting (Forg; $\downarrow$ indicates lower is better) for online augmented (labeled ``with DA'') EMR and Quadratic Regularization strategies (EWC, MAS, SI, RWalk, and Random) with Replay-based methods (A-GEM and ER-Reservoir). Due to space constraints, results for Vanilla regularizers are not provided. We consider three datasets: CIFAR-100 (10 tasks, labeled CIFAR); Oxford-Flowers (17 tasks, labeled Flowers); and Caltech-256 (32 tasks, labeled Cal-256). Best replay-based method's results are in bold. Best regularization-based method's results are underlined. As shown, the performance gap between online augmented EMR and replay-based methods is minimal. In contrast, \emph{existing} Quadratic Regularization strategies (except MAS) find it difficult to scale up when more updates are performed under online augmentation.}
\begin{tabular}{@{}c!{\vrule width 1pt}ccccc!{\vrule width 1pt}ccccc!{\vrule width 1pt}cc@{}}
\toprule
Dataset & \multicolumn{5}{c!{\vrule width 1pt}}{Quadratic Reg. (with DA)}         & \multicolumn{5}{c!{\vrule width 1pt}}{Explicit Movement Reg. (with DA)}                                 & \multicolumn{2}{c}{Replay} \\ \midrule
CIFAR   & EWC  & MAS  & SI   & RWalk & Rand & EWC        & MAS        & SI   & RWalk      & Rand       & A-GEM    & ER              \\ \midrule
Acc ($\uparrow$)    & 62.1 & 65.1 & 64.1 & 64.8  & 64.8 & 65.6       & {\ul 66.1} & 65.8 & 65.2       & 65.4       & 67.2     & \textbf{68.8}   \\
Forg ($\downarrow$)   & 4.68 & 1.04 & 8.22 & 0.86  & 0.27 & 0.40       & 0.46       & 0.53 & {\ul 0.21} & 0.23       & 1.29     & \textbf{0.69}   \\ \midrule
Flowers & EWC  & MAS  & SI   & RWalk & Rand & EWC        & MAS        & SI   & RWalk      & Rand       & A-GEM    & ER              \\ \midrule
Acc ($\uparrow$)    & 37.1 & 61.8 & 34.1 & 51.2  & 63.2 & 66.4       & 66.1       & 66.1 & 65.9       & {\ul 66.8} & 68.61    & \textbf{68.9}   \\
Forg ($\downarrow$)   & 22.1 & 4.72 & 18.1 & 12.5  & 2.42 & {\ul 0.68} & 1.31       & 1.15 & 1.34       & 0.81       & 4.08     & \textbf{3.45}   \\ \midrule
Cal-256 & EWC  & MAS  & SI   & RWalk & Rand & EWC        & MAS        & SI   & RWalk      & Rand       & A-GEM    & ER              \\ \midrule
Acc ($\uparrow$)    & 44.2 & 57.6 & 36.3 & 55.3  & 60.6 & 60.7       & {\ul 61.2} & 60.9 & 60.6       & 60.7       & 63.9     & \textbf{64.3}   \\
Forg ($\downarrow$)   & 8.42 & 2.97 & 13.3 & 4.10  & 0.89 & 0.45       & {\ul 0.16} & 0.47 & 0.54       & 0.48       & 2.89     & \textbf{2.75}   \\ \bottomrule
\end{tabular}
\end{table}
